Text Generation with Diffusion Language Models: A Pre-training Approach with Continuous Paragraph Denoise

In this paper, we introduce a novel dIffusion language modEl pre-training framework for text generation, which we call GENIE. GENIE is a large-scale pretrained diffusion language model that consists of an encoder and a diffusion-based decoder, which can generate text by gradually transforming a random noise sequence into a coherent text sequence. To pre-train GENIE on a large-scale language corpus, we design a new continuous paragraph denoise objective, which encourages the diffusion-decoder to reconstruct a clean text paragraph from a corrupted version, while preserving the semantic and syntactic coherence. We evaluate GENIE on four downstream text generation benchmarks, namely XSum, CNN/DailyMail, Gigaword, and CommonGen. Our experimental results show that GENIE achieves comparable performance with the state-of-the-art autoregressive models on these benchmarks, and generates more diverse text samples. The code and models of GENIE are available at https://github.com/microsoft/ProphetNet/tree/master/GENIE.

==> tables/main_result_gigaword.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{l|ccc}
\hline
\textbf{Method}  & \multicolumn{1}{l}{\textbf{ROUGE-1}} & \multicolumn{1}{l}{\textbf{ROUGE-2}} & \multicolumn{1}{l}{\textbf{ROUGE-L}} \\ \hline
LSTM~\cite{GreffSKSS17} & 34.2 & 16.0 & 31.8 \\
Transformer~\cite{VaswaniSPUJGKP17} & 37.1 & 18.4 & 34.5 \\
MASS~\cite{SongTQLL19} & 38.7 & 19.7 & 35.9 \\
ProphetNet~\cite{qi2020prophetnet} & 38.9 & 19.9 & 36.0 \\ \hline
\ours{} (w/o pre-train) & 43.7 & 23.3 & 40.8 \\
\ours{} & 45.2 & 25.3 & 42.3 \\ \hline
\end{tabular}
\caption{The main results on \textsc{Gigaword}.}
\label{tab:gigaword_result}
\end{table*}

==> tables/main_result_squadQG.tex <==
\begin{table*}[h]
\centering
\caption{Results of Semi-NAR, NAR and AR on \textsc{SQuAD v1.1}. Index \textbf{OVERALL} represents the average value of \textbf{ROUGE-L}, \textbf{BLEU-4} and \textbf{MTR}. It should be noted that \ours{} belongs to Semi-NAR.}
\small 
\begin{tabular}{llcccc}
\hline
 \textbf{Pattern} & \textbf{Methods} &  \multicolumn{4}{c}{\textbf{\textsc{SQuAD v1.1}}} \\                   
 &  & \textbf{ROUGE-L} & \textbf{BLEU-4} & \textbf{MTR} & \textbf{OVERALL}   \\ \hline                                    
%& BANG$_{large}$  &      &  & &  &  \\ \hline
\multirow{6}{*}{NAR}
& NAT~\cite{gu2017non}  &  31.5 & 2.5 & 8.9 & 14.3  \\ 
& iNAT~\cite{lee2018deterministic} &  32.4 & 2.3 & 8.8 & 14.5 \\ 
& CMLM~\cite{ghazvininejad2019mask} & 31.6 & 2.5 & 8.9 & 14.3 \\
& LevT~\cite{gu2019levenshtein} & 31.4 & 2.3 & 9.1 & 14.3   \\
&BANG~\cite{qi2021bang} & \textbf{44.1} & 12.8 & \textbf{19.0} &\textbf{25.3}  \\
&ELMER~\cite{DBLP:journals/corr/abs-2210-13304} & 40.2 & \textbf{13.5} & 20.1 & 24.6 \\ \hline
%&ProphetNet$_{large}$  & 35.78   & 11.20 & 30.09 & 25.69 &  32.95  \\
%&BANG$_{large}SCRATCH$  &  35.45  & 10.77 & 29.55 & 25.26 &  32.95  \\ \hline
%&BANG$_{large}CONTINUE$  &  35.45  & 10.77 & 29.55 & 25.26 &  32.95  \\ 
\multirow{6}{*}{AR}
%& Transformer~\cite{vaswani2017attention}  &     30.57 & 10.47 & 24.22  & 21.76 (+0.00) & 364.96 (22.9x)\\ 
& LSTM~\cite{GreffSKSS17} & 27.2 & 3.8 & 8.9 & 13.3 \\
& Transformer~\cite{vaswani2017attention} & 30.7 & 4.8 & 10.9 & 15.5  \\ 
% & Transformer large  &      &  & &  & 261.78 \\ 
% & Transformer large-3gram  &      &  & &  & 300.30 \\ 
& MASS~\cite{SongTQLL19} &   \textbf{49.4} &  20.1 & \textbf{24.4}  & 31.3   \\
& BART~\cite{lewis2019bart} & 42.6 & 17.1 & 23.2 & 27.6  \\
& ProphetNet~\cite{qi2020prophetnet} & 48.0 & 19.5 & 23.9  & 30.5  \\
& BANG~\cite{qi2021bang} & 49.3 & \textbf{21.4} & 24.3 & \textbf{31.7} \\

\hline
\multirow{7}{*}{Semi-NAR}
& InsT~\cite{stern2019insertion} & 30.0 & 2.3 & 8.2 & 13.5 \\ 
& iNAT~\cite{lee2018deterministic} & 32.3 & 3.2 & 9.2 & 14.9 \\ 
& CMLM~\cite{ghazvininejad2019mask} & 29.6 & 3.9 & 9.7 & 14.4 \\
& LevT~\cite{gu2019levenshtein} & 30.8 & 2.7 & 9.4 & 14.3 \\
& BANG~\cite{qi2021bang}  & \textbf{47.4} & 17.6 & 21.7 & 28.9 \\
&\ours{} (w/o pre-train) & 32.7 & 8.9 & 18.6 & 20.1 \\
&\ours{} &  44.7 & \textbf{20.5} & \textbf{27.4} & \textbf{30.9}\\ \hline



%&MASS$_{middle}$  &  39.1  & 16.5 & 31.4& 29 &  N/A  \\ 
%&BART$_{large}$  &   45.1 & 22.2 & 37.2 & 34.83  &  N/A  \\ 
%&ProphetNet$_{large}$  &44.4    & 21.3 & 36.4& 34.03 &  N/A  \\ 
%&BANG$_{large}SCRATCH$  & 43.47& 20.41 & 35.39  & 33.09 &  1052.63  \\ \hline
\end{tabular}
\label{table.result.SQUAD}
\end{table*}
